Prompt-aligned Gradient for Prompt Tuning

Thanks to the large pre-trained vision-language models (VLMs) like CLIP, we can craft a zero-shot classifier by "prompt", e.g., the confidence score of an image being "[CLASS]" can be obtained by using the VLM provided similarity measure between the image and the prompt sentence "a photo of a [CLASS]". Therefore, prompt shows a great potential for fast adaptation of VLMs to downstream tasks if we fine-tune the prompt-based similarity measure. However, we find a common failure that improper fine-tuning may not only undermine the prompt's inherent prediction for the task-related classes, but also for other classes in the VLM vocabulary. Existing methods still address this problem by using traditional anti-overfitting techniques such as early stopping and data augmentation, which lack a principled solution specific to prompt. We present Prompt-aligned Gradient, dubbed ProGrad, to prevent prompt tuning from forgetting the the general knowledge learned from VLMs. In particular, ProGrad only updates the prompt whose gradient is aligned (or non-conflicting) to the "general direction", which is represented as the gradient of the KL loss of the pre-defined prompt prediction. Extensive experiments demonstrate the stronger few-shot generalization ability of ProGrad over state-of-the-art prompt tuning methods. Codes are available at https://github.com/BeierZhu/Prompt-align.

==> tables/base2new.tex <==
\setlength{\intextsep}{5pt}%
\setlength{\columnsep}{5pt}%
\begin{wraptable}{r}{0.25\textwidth}
    \makeatletter\def\@captype{table}
    \tabstyle{3pt}
    \caption{Averaged accuracy (\%) over 11 datasets for base-to-new generalization.}
    \label{tab:results_generalization}
    \centering
    % \scalebox{0.9}{
    \begin{tabular}{l cc|c}
    \toprule
    & Base & New & H. \\
    \midrule
    CLIP &61.72 & 65.91 &63.64  \\
    CoOp & 71.96 &61.26 & 65.58 \\
    CoCoOp &72.23  &60.77 & 65.35  \\
    \rowcolor{tabhighlight}
    \texttt{ProGrad} & \textbf{73.29} & \textbf{65.96} & \textbf{69.06} \\
    \bottomrule
    \end{tabular}
    % }
\end{wraptable}


